An Empirical Study of False Negatives and Positives of Static Code Analyzers From the Perspective of Historical Issues

Static code analyzers are widely used to help find program flaws. However, in practice the effectiveness and usability of such analyzers is affected by the problems of false negatives (FNs) and false positives (FPs). This paper aims to investigate the FNs and FPs of such analyzers from a new perspective, i.e., examining the historical issues of FNs and FPs of these analyzers reported by the maintainers, users and researchers in their issue repositories -- each of these issues manifested as a FN or FP of these analyzers in the history and has already been confirmed and fixed by the analyzers' developers. To this end, we conduct the first systematic study on a broad range of 350 historical issues of FNs/FPs from three popular static code analyzers (i.e., PMD, SpotBugs, and SonarQube). All these issues have been confirmed and fixed by the developers. We investigated these issues' root causes and the characteristics of the corresponding issue-triggering programs. It reveals several new interesting findings and implications on mitigating FNs and FPs. Furthermore, guided by some findings of our study, we designed a metamorphic testing strategy to find FNs and FPs. This strategy successfully found 14 new issues of FNs/FPs, 11 of which have been confirmed and 9 have already been fixed by the developers. Our further manual investigation of the studied analyzers revealed one rule specification issue and additional four FNs/FPs due to the weaknesses of the implemented static analysis. We have made all the artifacts (datasets and tools) publicly available at https://zenodo.org/doi/10.5281/zenodo.11525129.

==> Sections/Statistical_analysis.tex <==
\section{Statistical analysis and data processing}
\label{sec:statis}
In this section, we give a macroscopic view of false negatives and false positives raised by the three Static code analyzers with statistical analysis and data processing.
\begin{table}[htbp]
  \centering
  \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{ccccc}
      \toprule
      Tool               & Total Java Rules & Issue related Rules & Issues & Issues per Rule \\
      \midrule
      \textsc{PMD}       & 325              & 101                 & 223    & 2.21            \\
      \textsc{SpotBugs}  & 468              & 16                  & 21     & 1.31            \\
      \textsc{SonarQube} & 618              & 64                  & 86     & 1.34            \\
      \bottomrule
    \end{tabular}%
  }
  \caption{Tool comparison}
  \label{tab:comparison}%
\end{table}%

As shown in table \ref{tab:comparison}, the average number of issues per rule for the three tools is between 1.31 and 2.21. However, the tools with higher ranks have significantly more issues than the average number of issues per rule for each tool.

\textbf{DIFFERENCE OF THESE THREE TOOLS}

\begin{table}[h]
  \centering

  \label{tab:pmdtop}
  \begin{tabular}{|l|r|}
    \hline
    \textbf{Rule}                 & \textbf{Issue Count} \\
    \hline
    ImmutableField                & 12                   \\
    \hline
    UnnecessaryFullyQualifiedName & 11                   \\
    \hline
    CloseResource                 & 11                   \\
    \hline
    UnusedPrivateField            & 8                    \\
    \hline
    UnusedImports                 & 8                    \\
    \hline
    InvalidLogMessageFormat       & 7                    \\
    \hline
    UnusedPrivateMethod           & 6                    \\
    \hline
    ArrayIsStoredDirectly         & 6                    \\
    \hline
    JUnitTestsShouldIncludeAssert & 5                    \\
    \hline
  \end{tabular}
  \caption{Top \textsc{PMD} Rules}
\end{table}

\begin{table}[h]
  \centering
  \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{|l|r|}
      \hline
      \textbf{Rule}                                 & \textbf{Issue Count} \\
      \hline
      DMI\_RANDOM\_USED\_ONLY\_ONCE                 & 2                    \\
      \hline
      NP\_NONNULL\_PARAM\_VIOLATION                 & 2                    \\
      \hline
      RV\_RETURN\_VALUE\_IGNORED                    & 2                    \\
      \hline
      RCN\_REDUNDANT\_NULLCHECK\_OF\_NONNULL\_VALUE & 2                    \\
      \hline
      UPM\_UNCALLED\_PRIVATE\_METHOD                & 2                    \\
      \hline
    \end{tabular}
  }
  \caption{\textsc{SpotBugs} Top Rules}
  \label{tab:spotbugstop}
\end{table}

S2589 \textit{Boolean expressions should not be gratuitous} failed because of the wrong resolution of \textsc{SonarQube}'s SE engine.
This rule in \textsc{SonarQube} is implemented with the SE engine, while the same function is implemented with pattern matching in \textsc{PMD}.

\begin{table}[h]
  \centering

  \label{tab:sonartop}
  \begin{tabular}{|l|r|}
    \hline
    \textbf{Rule} & \textbf{Issue Count} \\
    \hline
    s2589         & 3                    \\
    \hline
    s3749         & 3                    \\
    \hline
    s2384         & 3                    \\
    \hline
    s2259         & 3                    \\
    \hline
  \end{tabular}
  \caption{Top \textsc{SonarQube} Issues}
\end{table}


==> Sections/Workflow.tex <==
\section{workflow of static code analyzer}
\label{sec:workflow of static code analyzer}



A common workflow of a static code analyzer can be summarized as two stages: Process the source code (\textsc{PMD} and \textsc{SonarQube}) or byte code (\textsc{SpotBugs}) and execute rules. Figure \ref{fig:workflow} shows the common workflow of the static code analyzer.


\begin{figure*}[htbp]
    \centerline{\includegraphics[scale=0.58]{Figures/flowchart2.pdf}}
    \caption{Common workflow of static code analyzer}
    \label{fig:workflow}
\end{figure*}



Parse the source code and run visitors to get information in intermediate representation (\eg, abstract syntax tree)

Visitors build necessary information like scopes, dataflow and control flow relations. Different visitors provide different abilities to implement rules. For instance, \textsc{SpotBugs} is able to perform interprocedural analysis to a certain extent; \textsc{SonarQube}'s Symbolic Execution engine provides the ability to implement more rules like finding divide by zero, and null pointer dereference.

Using the provided information to match pre-defined bug patterns.

Both stages of the two steps may become the reason that produces false negatives and false positives.

These three analyzers have their own characteristics.

\textsc{SonarQube} provides deep analysis of code through symbolic execution, path-sensitive analysis \& cross-function/cross-file analysis.

SpotBugs construct diverse intermediate representations and implement dataflow analysis to achieve interprocedural analysis.

\textsc{PMD} do not have a general well-performed core module to perform common interprocedural analysis as well as cross-file analysis. The dataflow analysis module has been removed in the latest version of \textsc{PMD} 7. \textsc{PMD} uses pattern matching instead, focusing on the predefined rules.
\textsc{PMD} implements a stronger type resolution framework to implement rules in a precise and fast way. It also provides a feature-rich and pratical developer tool \textit{pmd-designer} to dump abundant information for implementing rules. Additionally, \textsc{PMD} supports implementing rules by XPath, which is friendly to learn and use.
